Algorithmic Decorrelation and Planted Clique in Dependent Random Graphs: The Case of Extra Triangles

We aim to understand the extent to which the noise distribution in a planted signal-plus-noise problem impacts its computational complexity. To that end, we consider the planted clique and planted dense subgraph problems, but in a different ambient graph. Instead of Erd\H{o}s-R\'enyi $G(n,p)$, which has independent edges, we take the ambient graph to be the random graph with triangles (RGT) obtained by adding triangles to $G(n,p)$. We show that the RGT can be efficiently mapped to the corresponding $G(n,p)$, and moreover, that the planted clique (or dense subgraph) is approximately preserved under this mapping. This constitutes the first average-case reduction transforming dependent noise to independent noise. Together with the easier direction of mapping the ambient graph from Erd\H{o}s-R\'enyi to RGT, our results yield a strong equivalence between models. In order to prove our results, we develop a new general framework for reasoning about the validity of average-case reductions based on low sensitivity to perturbations.

==> outline-notes.tex <==
\begin{itemize}
    \item There has been a recent focus on the computational limit of statistical problems.
    \item Average case reduction has been one of the approaches to understand the relation between different statistical problems. discuss how reduction is bread and butter of complexity theory and cryptography for good reason. gives a style of result that is much deeper than hardness against class of algorithms. (literatures)
    \item One limitation of the current literature in average case reduction is the lack of both-way equivalence. Most reductions are based on one computational hardness assumption. (introduce PC) (mention also reduction from LPN, hardness based on cryptographic assumptions, etc. --- see Amit Daniely. Daniel Kane. etc.)
    % \item (Possible) Another limitation is the limitation on the structure of the hidden signal.
    \item What is missing from the technical side? Existing reductions always reduce models with independent noise to models with dependent noise. One major technical barrier is ways to remove dependence in noise. 
\end{itemize}


\gb{It'd be good to also extend to rank 1 signal. I.e. subgraph stochastic block model. seems like all we need is to be able to ``plant" edge with \emph{smaller} probability than $p$ and commute with $\cA$}

\gb{It'd be good to extend to larger planted subgraph that has a smaller q}
